Illicit Darkweb Classification via Natural-language Processing: Classifying Illicit Content of Webpages based on Textual Information

This work aims at expanding previous works done in the context of illegal activities classification, performing three different steps. First, we created a heterogeneous dataset of 113995 onion sites and dark marketplaces. Then, we compared pre-trained transferable models, i.e., ULMFit (Universal Language Model Fine-tuning), Bert (Bidirectional Encoder Representations from Transformers), and RoBERTa (Robustly optimized BERT approach) with a traditional text classification approach like LSTM (Long short-term memory) neural networks. Finally, we developed two illegal activities classification approaches, one for illicit content on the Dark Web and one for identifying the specific types of drugs. Results show that Bert obtained the best approach, classifying the dark web's general content and the types of Drugs with 96.08% and 91.98% of accuracy.

==> sections/5_Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The results presented in the previous section will be discussed in this section. Moreover, we comment on the limitation of the study.\\

\noindent \textbf{Comments on Results.}
Previous research on the Dark Web content utilized textual information from limited data sources. In this paper, we extracted HTML pages from several marketplaces and sources. The highest accuracy score for the general Dark Web content achieved is 96.08\%. Looking at the paper of Graczyk \etal  \cite{Graczyk2015AutomaticPC}, they achieved 79\% of accuracy score but using only one marketplace, thus possibly making their result limited. So, we believe that combining textual information from different marketplaces and expanding the classification labels can achieve good results. 
Our study also considered different NLP techniques (\eg Bert), comparing them and finally providing two different classification approaches, one for illicit activity and one for types of drugs.
As shown in Section \ref{sec:results}, the performance of Bert and RoBERTa models achieved the best performance. This was true for the results generated from unseen data and examining the metrics scores. However, looking at the confusion matrix, Bert seems the best approach for both the tasks: classifying the entire dark web content and classifying the types of Drugs. 
To summarize, this paper employed various NLP approaches to classify illegal activities on the Dark Web, and succeeded in classifying the Dark Web illicit activities with 96.08\% accuracy. Furthermore, it can classify drug-related illicit activities to the specific types of drugs with 91.98\% accuracy.\\

\noindent \textbf{Previous Studies.}
The results of this research further expand the contributions of the previous studies. In particular, the Graczyk \etal \cite{Graczyk2015AutomaticPC} classified the illicit activities in the Agora marketplace with 79\% accuracy. According to Section \ref{sec:results} our paper achieved 96.08\% accuracy for classifying illegal activities for more than one marketplace, thus improving the classification of illicit content by adding more data sources. Furthermore, this study builds on existing evidence from the work of Al Nabki \etal \cite{ClassifyingIllegal} that illicit Dark Web content can be classified with high accuracy results. They divided and classified the illegal content only into four categories. This paper provides two types of classification tasks, \ie general content on the Dark Web (19 classes) and specific types of Drugs (49 classes). These additions provide new and improved classification approaches to illicit actions on the Dark Web.\\

\noindent \textbf{Limitations.}
A significant challenge in text classification tasks is developing models that apply to any language. The language issue is prevalent in all dark web studies. To the best of our knowledge, there are no studies that provided multilingual text classification approaches. A multilingual text classifier could understand the text from multiple languages.

Another challenge this study faced was the computing power or resources needed for executing the research models. This research explores the effects of transferable models such as Bert and RoBERTa. However, pre-trained models require vast computing resources to train from scratch and fine-tune them. As a result, the training of the models was limited by the available resources, thus possibly affecting results.

Lastly, the labeling and collection procedures of the data proved demanding. It was important for this research to generate a dataset from various Dark Web content sources. However, this process required much time, possibly affecting the instances obtained. However, these steps were manually double-checked by the authors of the paper.


% \section{Discussion}
% \label{sec:discussion}
% In this section, the results presented in the previous section will be discussed. First of all, the research questions established in the Introduction chapter will be answered using the results. Secondly, this research will be compared at a high level with previous studies. Thirdly, the limitations that appeared during the research will be examined. Finally, the possible future improvements and additional research based on this study are reviewed.

% \subsection{Research Questions}
% As a basis for this research, the following research question is posed: \textit{To what extent can illicit content and behavior from Dark nets pages be classified appropriately using various Natural Language Processing and Machine learning techniques?}. The answers to the five sub-questions will be investigated first to evaluate whether the central question is answered. These answers are then combined to determine the answer to the main research question.  

% The first sub-question this research addressed is: \textit{Is it possible to achieve state of the art results when combining textual information from pages belonging to different marketplaces?} 
% Previous research on the Dark Web content has utilized textual information from limited data sources, meaning onion sites from one marketplace. In this research indeed HTML pages from several marketplaces and sources have been utilized. The highest accuracy score for the general Dark Web content achieved is 96.08\%. To answer the first sub-question, this accuracy score could be compared with a different study that only utilized one data source. Specifically, in \cite{Graczyk2015AutomaticPC} the authors achieved 79\% accuracy score, but they had used data from only one marketplace, which makes their results limited. Considering that this research created 19 different classes, the generated classifier outperforms the one in \cite{ClassifyingIllegal}. As a result, the answer to the first sub-question is positive since this research managed to combine textual information from different marketplaces, expand the classification labels, and still achieve good results. 

% The second sub-question refers to the abilities of the pre-trained model, and its exact formulation is the following: 
% \textit{To what extend can transfer learning models surpass a traditional one in classifying illicit activities?} During this study, three transferable models have been utilized, particularly Bert, RoBERTa, and ULMFit to be compared with an LSTM model.
% Table \ref{table:results_main} and \ref{table:results_drugs} present the results for each model. According to the analysis in the Results chapter, the RoBERTa, Bert, and the ULMFit models surpass the LSTM model when classifying the general Dark Web content. Nonetheless, in the Drugs types classification task, the ULMFit model performs poorly and thus underperforms compared to the LSTM. All in all, two of the transferable models are established as the leading approaches. Consequently, transfer learning models can outperform traditional methods such as LSTM neural networks. 

% Moving on to the third sub-question subject, all the models mentioned above have been utilized in also creating Drugs Classes classifiers. The third sub-question that has been addressed is:
% \textit{Can the illicit activities related to drugs be further classified to the many different types of drugs?} To answer this sub-question, this research created 49 labels related to the types of drugs that can be found in table \ref{table:drugs_subclass}. Furthermore, four different models were trained on the Drugs Classes data, and according to the results in table \ref{table:results_drugs}, three of them achieved above 90\% accuracy. Therefore it is safe to claim that illicit activities explicitly related to Drugs were successfully divided and classified into their corresponding classes.

% The fourth sub-question addressed in this research is:
% What text classifying architectures present the best results with fewer data instances? This sub-question is answered by assessing the performance of the models on the general content in the Dark Web and the specific types of Drugs. According to the analysis in the Results chapter, the RoBERTa and the Bert methods were the least affected by the change in the size of the data. In more detail, a comparison between the results presented in table \ref{table:results_main} and \ref{table:results_drugs} concludes that the performance of the ULMFit model is mostly affected. In contrast, the other models still generate adequate scores.  

% For the last sub-question: \textit{Which classifying method performs the tasks best?} all the models created from the four primary methods are evaluated. In the Results chapter, the performance of the models during training is analyzed, and Bert and RoBERTa were deemed as best. Also, the results generated from unseen data are discussed for every model and every task. By examining the metrics scores from the testing of the models, Bert and RoBERTa again performed both tasks best. Following this to determine the overall best model, the confusion matrices were presented for Bert and RoBERTa. This last analysis resulted in Bert being the best approach for both classification tasks, namely, classifying the entire dark web content and classifying the types of Drugs. 

% The findings from the above sub-questions are combined to answer the central question: \textit{To what extent can illicit content and behavior from Dark nets pages be classified appropriately using various Natural Language Processing and Machine learning techniques?} Firstly, this study employed various NLP approaches to classify illegal activities on the Dark Web. Secondly, all these various methods managed to generate a high metrics score. Consequently, this study succeeded in classifying the Dark Web illicit activities with 96.08\% accuracy. Furthermore, it was able to further classify drug-related illicit activities to the specific types of drugs with 91.98\% accuracy.



% \subsection{Previous Studies}
% The results of this research further expand the contributions of the previous studies. In particular, the authors of \cite{Graczyk2015AutomaticPC} manage to classify the illicit activities in the Agora marketplace with 79\% accuracy. According to the Results chapter, this research achieved 96.08\% accuracy for classifying illegal activities for more than one marketplace. Consequently, this research improved the classification of illicit content by adding more data sources and surpassing \cite{Graczyk2015AutomaticPC} in accuracy scores. Furthermore, this study builds on existing evidence from \cite{ClassifyingIllegal} that the illicit Dark Web content can be classified with high accuracy results. The researchers of \cite{ClassifyingIllegal} have divided and classified the illegal content only in four categories. This research, on the other hand, has created two different classification tasks. Firstly, a model is utilized to analyze the general content on the Dark Web that is divided into 19 different classes. Secondly, a classifier dedicated to specific types of Drugs, precisely 49 types, is utilized. These additions provide a new and improved classification approach of the illicit actions in the Dark Web.

% \subsection{Limitations}
% A significant challenge in text classification tasks is developing models that apply to any language. The language issue is prevalent in all the previous studies in the Dark Web that dealt with the text. To this research's knowledge, no Dark Web study has created multilingual text classification approaches. Consequently, the limitation of establishing multilingual text classification methods for the Dark Web applies to this research. A multilingual text classifier can understand text from multiple languages. Unfortunately, such a model has not been developed in this research, and this affects its generalization. All the research methods in this study are able to understand only the English language, and thus they are limited to HTML pages written in that one language.

% Another challenge this study faced is related to the computing power or resources needed for executing the research models. In this research, the effects of transferable models such as Bert and RoBERTa are explored. However, pre-trained models, particularly the ones mentioned earlier, require vast computing resources not only for training them from scratch but even for fine-tuning them. As a result, the training of the models was limited by the available resources at hand. It is possible that with more considerable computing resources, the performance of the pre-trained models could be improved.

% Lastly, labeling and collection procedures of the data proved demanding. It was important for this research to generate a dataset from a variety of Dark Web content sources. While this objective was, in a sense, achieved, there were many limitations during the collection and labeling of the sites that proved time-consuming. 

% \subsection{Future Work}
% This research intended to experiment with pre-trained models and compare their performance to an LSTM model made from scratch. All the models are evaluated on two classification tasks, one regarding the general content of the Dark Web and another one specified to the types of drugs. Future work can built on many of this research's elements to improve the investigation of the Dark Web's content.

% First of all, new research can invest in cultivating a hierarchical classification model. This research created a drugs classifier as an attempt to mimic a class hierarchy. If an HTML page is classified as Drugs, then the drugs classifier determines the exact type of drug. It would be profitable to develop a text classification model that could hierarchically assign labels on the input. Meaning that if an onion page is given the label Services, then it would be useful to detect the specific service described on that page. 

% Secondly, the pre-trained models used in this research have been developed from their creators for a vast array of tasks. These models have been utilized in the past in tasks such as question and answering, next sentence prediction, sentiment analysis, and many more. Following this, future research can expand on this study and take advantage of the pre-trained models' ability to perform different tasks. More specifically, create a model that examines the textual content of the Dark Web in different ways. In particular, text from Dark Web forums can be analyzed with regard to sentiment.  

% Another future step can be to build on the existing text classification models and develop a multilingual model. The Bert model creators have released a multilingual approach, and according to \cite{multilingual} it manages to work well between similar languages. Consequently, since the transferable models achieved respectable results in this study compared to the LSTM model, further research can focus on developing a multilingual Bert model for the Dark Web content. This extension can be significant since every HTML, regardless of the language it is written, could be analyzed. 

% Lastly, while this research included many different data sources, it would still be beneficial to add more. In this study, data from many marketplaces and random hidden services from the Dark Web as well as illicit sites from the Normal Web have been used. Nonetheless, the content of these sources often changes; thus, continuous research on the Dark Web content is needed. Specifically, when unseen categories surface, then the models should be re-trained on them.   
